Instructify: Demystifying Metadata to Visual Instruction Tuning Data Conversion

Visual Instruction Tuning (VisIT) data, commonly available as human-assistant conversations with images interleaved in the human turns, are currently the most widespread vehicle for aligning strong LLMs to understand visual inputs, converting them to strong LMMs. While many VisIT datasets are available, most are constructed using ad-hoc techniques developed independently by different groups. They are often poorly documented, lack reproducible code, and rely on paid, closed-source model APIs such as GPT-4, Gemini, or Claude to convert image metadata (labels) into VisIT instructions. This leads to high costs and makes it challenging to scale, enhance quality, or generate VisIT data for new datasets. In this work, we address these challenges and propose an open and unified recipe and approach,~\textbf{\method}, for converting available metadata to VisIT instructions using open LLMs. Our multi-stage \method features an efficient framework for metadata grouping, quality control, data and prompt organization, and conversation sampling. We show that our approach can reproduce or enhance the data quality of available VisIT datasets when applied to the same image data and metadata sources, improving GPT-4 generated VisIT instructions by ~3\% on average and up to 12\% on individual benchmarks using open models, such as Gemma 2 27B and LLaMa 3.1 70B. Additionally, our approach enables effective performance scaling - both in quantity and quality - by enhancing the resulting LMM performance across a wide range of benchmarks. We also analyze the impact of various factors, including conversation format, base model selection, and resampling strategies. Our code, which supports the reproduction of equal or higher-quality VisIT datasets and facilities future metadata-to-VisIT data conversion for niche domains, is released at https://github.com/jacob-hansen/Instructify.

==> figure_tex/supp_prompt_shikra.tex <==
\begin{figure*}[ht]
% \vspace{-0.3cm}
\centering
\includegraphics[width=0.95\linewidth]{figures/supp_prompt_shikra.pdf}
\caption{
\label{fig:prompt_shikra}
\textbf{Shikra prompt.}
}
\end{figure*}

==> figures/results.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Master Table of Results across Benchmarks, Models, and Datasets}
    \label{tab:master-results}
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model/Dataset} & \textbf{AI2D} & \textbf{ChartQA} & \textbf{DocVQA} & \textbf{InfoVQA} & \textbf{SeedBench} & \textbf{MME} & \textbf{RealWorldQA} & \textbf{ScienceQA} & \textbf{TextVQA} \\ \hline
        GPT-4 & 0.628 & 0.177 & 0.454 & 0.326 & 0.692 & 321.78 & 0.573 & 0.783 & 0.562 \\ \hline
        Gemma 2 27B & 0.625 & 0.194 & 0.531 & 0.335 & 0.687 & 347.14 & 0.592 & 0.776 & 0.570 \\ \hline
        LLaMa 3.1 & 0.627 & 0.186 & 0.481 & 0.324 & 0.690 & 310.35 & 0.591 & 0.760 & 0.566 \\ \hline
    \end{tabular}
\end{table*}




==> prompts/docowl.tex <==
% DocOwl
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=DocOwl]
\small
You are an AI document analysis assistant examining a text-rich image through provided descriptions. Respond as if directly viewing the image.
Create a Q\&A dialogue that demonstrates understanding of: \\
- Core content and organization \\
- Visual structure and elements \\
- Relationships between components \\
- Quantitative aspects where relevant \\
 \\
Questions should: \\
- Be clearly answerable from the content \\
- Span multiple complexity levels \\
- Include synthesis tasks \\
- Focus on connections between elements \\
 \\
Answers should: \\
- Show step-by-step reasoning when applicable \\
- Paraphrase rather than quote \\
- Break down complex analysis \\
- Use natural language \\
 \\
Critical Instruction:  \\
- The dialogue length should match the depth and complexity of the provided content, without fabricating additional details. Sometimes this means the dialogue will be short. \\
- To avoid errors that occur in ocr, never directly quote text from the document. Instead, paraphrase and describe content in your own words. \\
 \\
Format the question/answer pairs as follows, with no introduction or explanation: \\
Question: [Question] \\
Answer: [Answer] \\
Question: [Question] \\
Answer: [Answer] \\
etc.
\end{tcolorbox}


==> prompts/llava.tex <==
% LLaVA Complex Reasoning
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=LLaVA Complex Reasoning]
\small
You are an AI visual assistant that can analyze a single image. You receive five sentences, each describing the same image you are observing. In addition, specific object locations within the image are given, along with detailed coordinates. These coordinates are in the form of bounding boxes, represented as (x1, y1, x2, y2) with floating numbers ranging from 0 to 1. These values correspond to the top left x, top left y, bottom right x, and bottom right y.
\\ \\
The task is to use the provided caption and bounding box information, create a plausible question about the image, and provide the answer in detail.
\\ \\
Create complex questions beyond describing the scene.
To answer such questions, one should require first understanding the visual content, then based on the background knowledge or reasoning, either explain why the things are happening that way, or provide guides and help to user's request. Make the question challenging by not including the visual content details in the question so that the user needs to reason about that first.
\\ \\
Instead of directly mentioning the bounding box coordinates, utilize this data to explain the scene using natural language. Include details like object counts, position of the objects, relative position between the objects.
\\ \\
When using the information from the caption and coordinates, directly explain the scene, and do not mention that the information source is the caption or the bounding box. Always answer as if you are directly looking at the image.
\\ \\
Avoid extrapolation or making assumptions about the image content. Only answer based on the information provided in the image.
Format the question/answer pair as follows, with no introduction or explanation:\\
Question: [Question]  \\
Answer: [Answer]
\end{tcolorbox}

% LLaVA Conversation
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=LLaVA Conversation]
\small
You are an AI visual assistant, and you are seeing a single image. What you see are provided with five sentences, describing the same image you are looking at. Answer all questions as you are seeing the image.
\\ \\
Design a conversation between you and a person asking about this photo. The answers should be in a tone that a visual AI assistant is seeing the image and answering the question.  \\
Ask diverse questions and give corresponding answers.
\\ \\
Include questions asking about the visual content of the image, including the object types, counting the objects, object actions, object locations, relative positions between objects, etc. Only include questions that have definite answers:  \\
(1) One can see the content in the image that the question asks about and can answer confidently.  \\
(2) One can determine confidently from the image that it is not in the image.  
Do not ask any question that cannot be answered confidently.
\\ \\
Also include complex questions that are relevant to the content in the image, for example, asking about background knowledge of the objects in the image, asking to discuss events happening in the image, etc. Again, do not ask about uncertain details.  \\
Provide detailed answers when answering complex questions. For example, give detailed examples or reasoning steps to make the content more convincing and well-organized. You can include multiple paragraphs if necessary.
\\ \\
Avoid extrapolation or making assumptions about the image content. Only answer based on the information provided in the image. \\ 
Format the question/answer pairs as follows, with no introduction or explanation: \\
Question: [Question]  \\
Answer: [Answer]  \\
Question: [Question]  \\
Answer: [Answer]
\end{tcolorbox}

% LLaVA Detail
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=LLaVA Detail]
\small
You are an AI visual assistant that can analyze a single image. You receive five sentences, each describing the same image you are observing. In addition, specific object locations within the image are given, along with detailed coordinates. These coordinates are in the form of bounding boxes, represented as (x1, y1, x2, y2) with floating numbers ranging from 0 to 1. These values correspond to the top left x, top left y, bottom right x, and bottom right y.
\\ \\
Using the provided caption and bounding box information, describe the scene in a detailed manner.
\\ \\
Instead of directly mentioning the bounding box coordinates, utilize this data to explain the scene using natural language. Include details like object counts, position of the objects, relative position between the objects.
\\ \\
When using the information from the caption and coordinates, directly explain the scene, and do not mention that the information source is the caption or the bounding box. Always answer as if you are directly looking at the image.
\\ \\
Avoid extrapolation or making assumptions about the image content. Only answer based on the information provided in the image. \\
Format the question/answer pair as follows, with no introduction or explanation: \\
Question: [Question]  \\
Answer: [Answer]
\end{tcolorbox}

==> prompts/llavar.tex <==
% LLaVAR
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=LLaVAR]
\small
You are an AI visual assistant, and you are seeing a single image. What you see is provided with two OCR results and one image caption describing the information within the same image you are looking at. Image captions might include hallucinations, while OCR results are more accurate. Answer all questions with definite answers as you are seeing the image.
 \\ \\
Design a conversation between you and a person asking about this photo. The answers should be in a tone that a visual AI assistant is seeing the image and answering the question. Ask diverse questions and give corresponding answers. Include questions asking about the visual content of the image (e.g., the man, the sunset, the ocean) and the texts contained in the image. Only include questions that have definite answers: \\
(1) One can see the content in the image that the question asks about and can answer confidently;   \\
(2) One can determine confidently from the image that it is not in the image;   \\
(3) DO NOT mention OCR or image caption in your questions and answers; \\
(4) DO NOT ask about information from captions while it looks unrelated to or contradicts OCR results;   \\
(5) Correct any obvious OCR text errors and formatting mistakes by making sense of what information is present. Use proper capitalization, spacing, and spelling that likely reflects how the text actually appears in the image. \\
 \\
Also include complex questions that are relevant to the content in the image, for example, asking about background knowledge of the texts in the image, asking to discuss about the design of the image, etc. Again, do not ask about uncertain details. Provide detailed answers when answering complex questions. For example, give detailed examples or reasoning steps to make the content more convincing and well-organized. You can include multiple paragraphs if necessary.
 \\ \\
Format the question/answer pairs as follows, with no introduction or explanation: \\
Question: [Question]   \\
Answer: [Answer]   \\
Question: [Question]   \\
Answer: [Answer]
\end{tcolorbox}

==> prompts/lvis.tex <==
% LVIS Conversation
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=LVIS Conversation]
\small
You are an AI visual assistant, and you are seeing a single image. Answer all questions as you are seeing the image. Design a conversation between you and a person asking about this photo. The answers should be in a tone that a visual AI assistant is seeing the image and answering the question. Ask diverse questions and give corresponding answers. Include questions asking about the visual content of the image, including the object types, counting the objects, object actions, object locations, relative positions between objects, etc. Only include questions that have definite answers: (1) one can see the content in the image that the question asks about and can answer confidently; (2) one can determine confidently from the image that it is not in the image. Do not ask any questions that cannot be answered confidently. Also include complex questions that are relevant to the content in the image, for example, asking about background knowledge of the objects in the image, asking to discuss events happening in the image, etc. Again, do not ask about uncertain details, but the questions should be challenging enough, requiring the person to utilize 1) complex reasoning; 2) world knowledge; 3) explanatory answers; and 4) multi-turn conversation, to give accurate answers. Please provide detailed answers when answering complex questions. For example, give detailed examples or reasoning steps to make the content more convincing and well-organized. Please ensure all the questions are closely related to the visual content of the provided image, which means that if the person cannot see the picture but only gets access to the text description of it, he/she will not be able to answer accurately. If the AI assistant asks counterfactual questions, the person should give a negative answer, rather than making up an answer. \\
 \\
Note, clothing mentioned may be being worn by people in the image. Do not assume things. \\
Avoid extrapolation or making assumptions about the image content. Only answer based on the information provided in the image. \\
Format the question/answer pairs as follows, with no introduction or explanation: \\
Question: [Question] \\
Answer: [Answer] \\
Question: [Question] \\
Answer: [Answer]
\end{tcolorbox}

% LVIS Detail
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=LVIS Detail]
\small
You are an AI visual assistant that can analyze a single image. When provided with information about an image, you will first create an appropriate broad question that could apply to any image (e.g., "What is happening in this scene?", "What do you observe in this image?", "Can you describe the main elements?"), then provide a precise and comprehensive answer that incorporates all the provided details. Your response should draw upon background knowledge and reasoning to either explain why things appear as they do or provide context that aids understanding. Focus solely on elements mentioned in the provided information, avoiding speculation about objects or details not explicitly stated. Answer as if you are directly observing the image, rather than working from a description. If addressing the task accurately becomes too challenging, please respond with [failed].
 \\ \\
Note, clothing mentioned may be being worn by people in the image.
Avoid extrapolation or making assumptions about the image content. Only answer based on the information provided in the image. \\
Format the question/answer pair as follows, with no introduction or explanation: \\
Question: [Question] \\
Answer: [Answer].
\end{tcolorbox}

==> prompts/polite_flamingo.tex <==
% Polite Flamingo
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=Polite Flamingo]
\small
You are an AI assistant that maintains the natural, helpful interaction style of large language models. Transform the provided information into a flowing conversation that bridges raw annotations and natural dialogue. \\
\\ \\
Essential Rules:   \\
1. Transform fragmentary information into complete, natural responses that preserve all facts.   \\
2. Use polite, helpful language with correct grammar and effective rhetoric.   \\
3. Provide appropriate elaboration while staying strictly grounded in what is known by the given information.   \\
4. Include clear answers followed by relevant supporting details and smooth transitions.   \\
5. Convert any technical details into natural observations about what is seen.   \\
6. Use observational language ("I can see...", "The image shows..."). \\  
7. When reasoning, provide clear rationales based only on given facts. \\
\\ \\
Format the conversation as follows (with no introduction): \\
Question: [Question]   \\
Answer: [Answer]   \\
Question: [Question]   \\
Answer: [Answer]
\end{tcolorbox}

==> prompts/shikra.tex <==
\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=Shikra Prompt]
\small
You are an AI visual assistant, and you are seeing a single image. What you see are provided with captions and bounding boxes of objects in the image. \\
 \\
Design a conversation between you and a person asking about this photo. The answers should be in a tone that a visual AI assistant is seeing the image and answering the question. Ask diverse questions and give corresponding answers. \\
 \\
\textless{}INSERTED\_CONVESATION\_FORMAT\textgreater{} \\
 \\
Include questions asking about the visual content of the image, including the object types, counting the objects, object actions, object locations, relative positions between objects, etc. Only include questions that have definite answers: \\
(1) one can see the content in the image that the question asks about and can answer confidently; \\
(2) one can determine confidently from the image that it is not in the image.
Do not ask any question that cannot be answered confidently. \\
 \\
Also include complex questions that are relevant to the content in the image, for example, asking about background knowledge of the objects in the image, asking to discuss about events happening in the image, etc. Again, do not ask about uncertain details. \\
Provide detailed answers when answering complex questions. For example, give detailed examples or reasoning steps to make the content more convincing and well-organized. You can include multiple paragraphs if necessary. \\
 \\
Format the question/answer pairs as follows, with no introduction or explanation: \\
Question: [Question] \\
Answer: [Answer] \\
Question: [Question] \\
Answer: [Answer] \\
etc.
\end{tcolorbox}


\begin{tcolorbox}[colback=gray!10, colframe=gray!40, sharp corners, title=Shikra Conversation Formats]
\small
\textbf{Spotting with Coordinates} \\
- Questions: Ask about scene contents with explicit requests for coordinates \\
- Answers: Describe objects/actions with precise locations [x1, y1, x2, y2]

\textbf{Grounding Caption} \\
- Questions: Query about specific regions using coordinates [x1, y1, x2, y2] \\
- Answers: Detailed descriptions of bounded regions

\textbf{REG (Referring Expression Generation)} \\
- Questions: Request unique descriptions of specific regions \\
- Answers: Provide distinctive features to differentiate regions

\textbf{Q→A (Question Answering)} \\
- Questions: Clear queries about visible contents/events \\
- Answers: Concise, factual responses based on visible elements

\textbf{Q→CA (Question with Careful Analysis)} \\
- Questions: Prompt for answers and reasoning \\
- Answers: Step-by-step logic and detailed visual evidence analysis

\textbf{Q→CBox A (Question with Coordinates Answer)} \\
- Questions: Open-ended scene content queries \\
- Answers: Natural descriptions with bounding boxes [x0,y0,x1,y1]
\end{tcolorbox}

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/jacob_notes_related_work.tex <==


\section{Related Work - Jacob's notes}
Works to mention:
Molmo and PixMo: (this is the work most similar to ours, here, they do the dirty work to actually collect the data and unify everything, but this was a huge efforts. There are 51 Authors! This reflects that the improvements are done through the careful work of so many people. We aim to accelerate this process on the assumption of already having collected data)
% Open Weights and Open Data for State-of-the-Art Multimodal Models
% We present Molmo, a new family of VLMs that are state-of-the-art in their class of openness. Our key innovation is a novel, highly detailed image caption dataset collected entirely from human annotators using speech-based descriptions. To enable a wide array of user interactions, we also introduce a diverse dataset mixture for fine-tuning that includes in-the-wild Q\&A and innovative 2D pointing data. The success of our approach relies on careful choices for the model architecture details, a well-tuned training pipeline, and, most critically, the quality of our newly collected datasets, all of which will be released. 


Math-LLaVA: (this is an example input work, where we repeat the prompt and experiment with it)
% To bridge this gap, we address the lack of high-quality, diverse multimodal mathematical datasets by collecting 40K high-quality images with question-answer pairs from 24 existing datasets and synthesizing 320K new pairs, creating the MathV360K dataset, which enhances both the breadth and depth of multimodal mathematical questions. We introduce MathLLaVA, a LLaVA-1.5-based model fine-tuned with MathV360K. This novel approach significantly improves the multimodal mathematical reasoning capabilities of LLaVA-1.5, achieving a 19-point increase and comparable performance to GPT-4V on MathVista’s minitest split, and yielding leading performance on Math-V and MathVerse. Furthermore, Math-LLaVA demonstrates enhanced generalizability, showing substantial improvements on the MMMU benchmark. Our research highlights the importance of dataset diversity and synthesis in advancing MLLMs’ mathematical reasoning abilities.


LLaVA: (this is the original llava-1.5 paper, we base a lot of our work from the dataset created here)
% In this paper, we present the first attempt to use language-only GPT-4 to generate multimodal language-image instruction-following data. By instruction tuning on such generated data, we introduce LLaVA: Large Language and Vision Assistant, an end-to-end trained large multimodal model that connects a vision encoder and LLM for general purpose visual and language this http URL early experiments show that LLaVA demonstrates impressive multimodel chat abilities, sometimes exhibiting the behaviors of multimodal GPT-4 on unseen images/instructions, and yields a 85.1% relative score compared with GPT-4 on a synthetic multimodal instruction-following dataset.


VILA2: (this is an example input work, where we repeat the prompt and experiment with it)
% Visual language models (VLMs) have rapidly progressed, driven by the success of
% large language models (LLMs). While model architectures and training infrastructures advance rapidly, data curation remains under-explored. When data quantity and quality become a bottleneck, existing work either directly crawls more raw data from the Internet that does not have a guarantee of data quality or distills from black-box commercial models (e.g., GPT-4V [1] / Gemini [2]) causing the performance upper bounded by that model. In this work, we introduce a novel approach that includes a self-augment step and a specialist-augment step to iteratively improve data quality and model performance. In the self-augment step, a VLM recaptions its own pretraining data to enhance data quality, and then retrains from scratch using this refined dataset to improve model performance. This process can iterate for several rounds. Once self-augmentation saturates, we employ several specialist VLMs finetuned from the self-augmented VLM with domain-specific
% expertise, to further infuse specialist knowledge into the generalist VLM through task-oriented recaptioning and retraining. With the combined self-augmented and specialist-augmented training, we introduce VILA2 (VILA-augmented-VILA), a VLM family that consistently improves the accuracy on a wide range of tasks over prior art, and achieves new state-of-the-art results on MMMU leaderboard [3] among open-sourced models.


Cambrian-1: (this is an example of a dataset that just aggregates the data, and not the works underneath, this is also a model that we rebuild and improve on, showing replacement of GPT-4 generated data)
% We introduce Cambrian-1, a family of multimodal LLMs (MLLMs) designed with a visioncentric approach. While stronger language models can enhance multimodal capabilities, the design choices for vision components are often insufficiently explored and disconnected from visual representation learning research. This gap hinders accurate sensory grounding in realworld scenarios. Our study uses LLMs and visual instruction tuning as an interface to evaluate various visual representations, offering new insights into different models and architectures— self-supervised, strongly supervised, or combinations thereof—based on experiments with over 20 vision encoders. We critically examine existing MLLM benchmarks, addressing the difficulties involved in consolidating and interpreting results from various tasks, and introduce a new vision-centric benchmark, CV-Bench. To further improve visual grounding, we propose the Spatial Vision Aggregator (SVA), a dynamic and spatially-aware connector that integrates high-resolution vision features with LLMs while reducing the number of tokens. Additionally, we discuss the curation of high-quality visual instruction-tuning data from publicly available sources, emphasizing the importance of data source balancing and distribution ratio. Collectively, Cambrian-1 not only achieves state-of-the-art performance but also serves as a comprehensive, open cookbook for instruction-tuned MLLMs. We provide model weights, code, supporting tools, datasets, and detailed instruction-tuning and evaluation recipes. We
% hope our release will inspire and accelerate advancements in multimodal systems and visual
% representation learning.

\subsection{Existing Datasets and Approaches}

\begin{itemize}
    \item \textbf{Datasets for Comparison:}
    \begin{itemize}
        \item Polite Flamingo \cite{polite_flamingo}
        \item LLaVA-RLHF\cite{llava_rlhf}
        \item mPLUG-DocOwl \cite{mplug_docowl}
        \item ShareGPT4V \cite{sharegpt4v}
        \item Shikra \cite{shikra}
        \item MACAW-LLM \cite{macaw_llm}
        \item LVIS-Instruct \cite{lvis_instruct}
        \item LRV-Instruct \cite{lrv_instruct}
        \item LLaVAR \cite{llavar}
        \item ALLaVA \cite{allava}
    \end{itemize}
\end{itemize}

\subsection{Limitations of Previous Works}

\begin{itemize}
    \item \textbf{Lack of Unification and Standardization:} Previous works typically focus on individual datasets, leading to fragmentation.
    \item \textbf{Closed-Source Codebases:} Many methods use proprietary code, which limits reproducibility.
    \item \textbf{Reliance on GPT-4:} The closed-source, expensive nature of GPT-4 constrains accessibility.
\end{itemize}

\subsection{Our Position}

Our work addresses these limitations by providing an open-source platform that unifies metadata from diverse datasets and enables scalable, repeatable synthetic data generation. This platform democratizes the ability to experiment with visual instruction tuning, reducing the need for closed-source models.

==> tables/llava_replacement.tex <==
\begin{table}[htbp]
\centering
\caption{Dataset Contributions to Captions, Bounding Boxes, and QA Tasks}
\label{tab:dataset_contributions}
\begin{tblr}
\hline
\textbf{Dataset Group} & \textbf{\# Images} & \textbf{\# Captions} & \textbf{\# Bounding Boxes} & \textbf{\# QA} \\
\hline
\hline
\multicolumn{5}{}{\textbf{Polite Flamingo}} \\
a\_ok\_vqa & 10,407 & 0 & 0 & 10,407\\
coco\_captions\_2014 & 79,866 & 399,513 & 583,502 & 0\\
dior\_rsvg & 8,866 & 0 & 39,644 & 0\\
flickr & 30,501 & 152,504 & 0 & 0\\
gqa & 80,356 & 0 & 6,201,642 & 900,764\\
hrrsd & 13,458 & 13,458 & 47,162 & 0\\
image2paragraph & 14,194 & 14,198 & 0 & 0\\
image\_editing\_request & 838 & 838 & 0 & 0\\
levir\_cc & 9,870 & 49,350 & 0 & 0\\
ocr\_vqa & 95,719 & 282,928 & 0 & 464,978\\
refcocog & 20,975 & 0 & 77,000 & 0\\
remoteclip\_ret3 & 13,408 & 81,888 & 0 & 0\\
scienceqa & 5,876 & 5,876 & 0 & 2,591,240\\
textcaps & 20,968 & 1,152,690 & 0 & 0\\
textvqa & 20,968 & 20,968 & 0 & 33,054\\
visual7w & 5,628 & 0 & 0 & 27,222\\
vqa\_e & 66,931 & 0 & 0 & 151,092\\
vqa\_v2 & 79,866 & 0 & 0 & 428,183\\
\hline[dashed]
Total & 373,920 & 2,174,211 & 6,948,950 & 4,606,940\\
\hline
\hline

\multicolumn{5}{}{\textbf{LLaVAR}} \\
llavar & 13,104 & 13,104 & 49,282 & 0\\
\hline[dashed]
Total & 1 & 13,104 & 49,282 & 0\\
\hline
\hline
\multicolumn{5}{}{\textbf{1x Mix}} \\
a\_ok\_vqa & 8,195 & 0 & 0 & 8,195\\
coco\_captions & 56,979 & 285,058 & 424,259 & 0\\
info\_vqa & 319 & 0 & 0 & 1,735\\
localized\_narratives & 56,979 & 64,983 & 0 & 0\\
lvis & 47,546 & 94,770 & 603,979 & 0\\
ocr\_vqa & 60,418 & 177,434 & 0 & 292,497\\
ok\_vqa & 4,514 & 0 & 0 & 4,514\\
refcoco & 8,692 & 0 & 61,943 & 0\\
refcocog & 11,092 & 0 & 40,827 & 0\\
refcocoplus & 8,691 & 0 & 61,810 & 0\\
text\_vqa & 11,497 & 11,497 & 0 & 18,138\\
textcaps & 11,497 & 631,955 & 0 & 0\\
visual7w & 7,484 & 0 & 0 & 36,333\\
visual\_genome & 55,951 & 0 & 3,169,962 & 0\\
vsr & 2,972 & 5,293 & 0 & 0\\
\hline[dashed]
Total & 160,643 & 1,270,990 & 4,362,780 & 361,412\\
\hline
\hline
\multicolumn{5}{}{\textbf{DocOwl}} \\
chart\_qa & 17,023 & 0 & 0 & 26,356\\
doc\_vqa & 8,675 & 0 & 0 & 43,963\\
docowl & 50,999 & 0 & 761,060 & 0\\
info\_vqa & 1,945 & 0 & 0 & 9,190\\
mm\_visualmrc & 2,796 & 0 & 0 & 11,016\\
text\_vqa & 20,561 & 20,561 & 0 & 32,426\\
\hline[dashed]
Total & 51,000 & 20,561 & 761,060 & 122,951\\
\hline
\hline
\hline
\multicolumn{5}{}{\textbf{Shikra}} \\
flickr & 14,923 & 74,614 & 0 & 0\\
refcoco & 4,638 & 0 & 31,218 & 0\\
refcocog & 6,487 & 0 & 22,756 & 0\\
refcocoplus & 4,638 & 0 & 31,245 & 0\\
visual7w & 1,929 & 0 & 0 & 9,791\\
visual\_genome & 15,480 & 0 & 469,580 & 0\\
vqa\_v2 & 25,947 & 0 & 0 & 142,076\\
\hline[dashed]
Total & 52,123 & 74,614 & 554,799 & 151,867\\
\hline
\hline

\end{tblr}
\label{tab:dataset_contributions}
\end{table}

==> tables/mytable2.tex <==
\begin{table*}[ht]
\scriptsize
\begin{tabular}{M{2cm}M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}M{1.5cm}cccccccccccccccccccc}
\toprule
Benchmarks & LLaVA & Our LLaVA & PF-1M & Our PF-1M & LLaVAR &  Our LLaVAR \\
\midrule
GQA        &     \\
TextVQA    &           &                            \\
ChartVQA   &           &                           \\
\bottomrule
\end{tabular}
\caption{In the ``Jacob-xx" experiments, there are the same number of points as original sets}
\label{tab:table2}
\end{table*}
